Acceleration of RANS Solver Convergence via Initialization with Wake Extension Models

Use of appropriate initialization to warm-start Reynolds-averaged Navier-Stokes (RANS) simulations of turbulent flow can facilitate convergence and lead to efficient use of computational resources. In this work, a method to model downstream wake development in external turbulent flow is proposed and used for RANS solver convergence acceleration. To balance the model accuracy and cost, the proposed method divides the analysis domain into three regions: near-body, wake and off-body. An approach based on a convolutional neural network is introduced as an efficient method to predict the downstream wake development. The model training only requires data from a single simulation, and its use is demonstrated to be effective in accelerating the RANS simulation when combined with an accurate flow prediction in the near-body region. The simulation using the proposed method took 26.3x fewer iterations, achieving 16.4x speedup in wall-clock time, compared to a baseline run using freestream initialization.

==> sections/math_commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATHEMATICAL DEFINITION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom Commands
%---------------------------------------------------------------------------
% Concise referencing
\newcommand{\eqnref}[1]{\eqref{#1}}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\figref}[1]{Figure \ref{#1}}
\newcommand{\lemref}[1]{Lemma \ref{#1}}
\newcommand{\corref}[1]{Corollary \ref{#1}}
\newcommand{\thmref}[1]{Theorem \ref{#1}}
% Real numbers
\newcommand{\Real}[1]{\mathbb{R}^{#1}}
\newcommand{\Complex}[1]{\mathbb{C}^{#1}}
\newcommand{\Integer}[1]{\mathbb{Z}^{#1}}
% Vec operator
\newcommand{\vecop}{\textnormal{vec}}
% Norm
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
% Absolute value 
\newcommand{\abs}[1]{\left|#1\right|}
% Parenthesis
\newcommand{\prt}[1]{\left(#1\right)}
% Trace
\newcommand{\trace}{\textnormal{tr}}
% Range
\newcommand{\range}{\textnormal{range}}
% Partial derivative
\newcommand{\pd}[2]{\dfrac{\partial #1}{\partial #2}}
% Complete derivative
\newcommand{\dd}[2]{\dfrac{d #1}{d #2}}
% Complete derivative, second order
\newcommand{\dds}[2]{\dfrac{d^2 #1}{d {#2}^2}}
% Limit to N / N
\newcommand{\limover}[1]{\lim_{#1 \rightarrow \infty} \dfrac{1}{#1}}
% Display style sum
\newcommand{\dsum}{\displaystyle\sum}
% arg min and arg max
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg~max}}}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg~min}}}

% degree
\newcommand{\dg}{$^\circ$}
% EIFs
\newcommand{\eifs}{\left(\Phi,\Psi,U\right)}

% Sampling pts
\newcommand{\sample}[1]{\{#1\}_{i=1}^{N_{p}}}
\newcommand{\eval}[1]{\{#1\}_{i=1}^{N_{e}}}
\newcommand{\Kcases}[1]{\{#1\}_{k=1}^{K}}

% potential flow
\newcommand{\plf}{p_{LF}}
\newcommand{\ulf}{u_{LF}}
\newcommand{\vlf}{v_{LF}}
% HF, LF and ML fields 
\newcommand{\qhf}{q}
\newcommand{\vecqhf}{\bm{q}}
\newcommand{\qlf}{q_{LF}}
\newcommand{\vecqlf}{\bm{q}_{LF}}
\newcommand{\qml}{\tilde{q}}
\newcommand{\vecqml}{\tilde{\bm{q}}}
\newcommand{\deltavecqml}{\delta{\tilde{\bm{q}}}}
\newcommand{\vecqfs}{\bm{q}_{FS}}
\newcommand{\vecqpofu}{\bm{q}_{POFU}}
% ML flow fields
\newcommand{\uml}{$\tilde{u}$}
\newcommand{\vml}{$\tilde{v}$}
\newcommand{\vecuml}{$\tilde{\bm{u}}$}
\newcommand{\absuml}{$\abs{\tilde{\bm{u}}}$}
\newcommand{\pml}{$\tilde{p}$}

\newcommand{\rhoml}{$\tilde{\rho}$}
\newcommand{\pxml}{$\tilde{p_{1}}$}
\newcommand{\pyml}{$\tilde{p_{2}}$}
\newcommand{\Eml}{$\tilde{E}$}
\newcommand{\rhoxnutildeml}{$\tilde{\rho}\times\tilde{\nu}$}
% Reynolds number
\newcommand{\Rey}{$Re$}
% Loss function
\newcommand{\lossl}{\mathcal{L}}
\newcommand{\lossldata}{\mathcal{L_{\rm{data}}}}
\newcommand{\losslgrad}{\mathcal{L_{\rm{grad}}}}

\newcommand{\nnorm}{\mathbf{n}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\atx}{\left(\x\right)}
\newcommand{\atxi}{\left(\x_{i}\right)}
%---------------------------------------------------------------------------
\newtheorem{theorem}{Theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

